Detection of Undeclared EV Charging Events in a Green Energy Certification Scheme

The green potential of electric vehicles (EVs) can be fully realized only if their batteries are charged using energy generated from renewable (i.e. green) sources. For logistic or economic reasons, however, EV drivers may be tempted to avoid charging stations certified as providing green energy, instead opting for conventional ones, where only a fraction of the available energy is green. This behaviour may slow down the achievement of decarbonisation targets of the road transport sector. In this paper, we use GPS data to infer whether an undeclared charging event has occurred. Specifically, we construct a Bayesian hypothesis test for the charging behaviour of the EV. Extensive simulations are carried out for an area of London, using the mobility simulator, SUMO, and exploring various operating conditions. Excellent detection rates for undeclared charging events are reported. We explain how the algorithm can serve as the basis for an incentivization scheme, encouraging compliance by drivers with green charging policies.

==> PaperBibliography.tex <==
@book{iea2023global,
  title={Global ev outlook 2023: Catching up with climate ambitions},
  author={IEA and AIE},
  year={2023},
  publisher={OECD Publishing}
}

@techreport{mckinsey2021,
    author = {McKinsey},
    institution = {McKinsey \& Company},
    title = {Scaling {EV} infrastructure to meet net-zero targets},
    year = {October 2021}
}

@techreport{allcost2024,
    institution = {Allstar Business Solutions},
    author = {All Star},
    title = {Revealing the real-life cost of petrol, diesel and electric},
    year = {Winter 2024}
}

@INPROCEEDINGS{10084262,
  author={M. H. Norouzi and M. Gholami and R. Noroozian},
  booktitle={2023 8th International Conference on Technology and Energy Management (ICTEM)}, 
  title={A comprehensive study of optimal demand management for a distributed network with the EV charging stations}, 
  year={2023},
  volume={},
  number={},
  pages={1-6},
  keywords={Vehicle-to-grid;Voltage;Power system stability;Charging stations;Air pollution;Electric vehicle charging;Fossil fuels;Electric vehicles (EVs);Green energy;Genetic algorithm (GA);Vehicle to grid(V2G);Distributed generations (DGs)},
  doi={10.1109/ICTEM56862.2023.10084262}}

@inproceedings{norouzi2023comprehensive,
  title={A comprehensive study of optimal demand management for a distributed network with the EV charging stations},
  author={M. H. Norouzi and M. Gholami and R. Noroozian},
  booktitle={2023 8th International Conference on Technology and Energy Management (ICTEM)},
  pages={1--6},
  year={2023},
  organization={IEEE},
  doi={10.1109/ICTEM56862.2023.10084262}
}

@article{krajzewicz2010traffic,
  title={Traffic simulation with SUMO--simulation of urban mobility},
  author={D. Krajzewicz},
  journal={Fundamentals of traffic simulation},
  pages={269--293},
  year={2010},
  publisher={Springer}
}

@article{Sponge,
  title={Smart procurement of naturally generated energy ({SPONGE}) for {PHEV}s},
  author={Y. Gu and F. H\"{a}usler and W. Griggs and E. Crisostomi and R. Shorten},
  journal={International Journal of Control},
  pages={1467--1480},
  year={2016},
  volume={89},
  number={7},
  publisher={Taylor \& Francis}
}

 @misc{OpenStreetMap,
   author = {{OpenStreetMap contributors}},
   title = {{Planet dump retrieved from https://planet.osm.org }},
   howpublished = "\url{ https://www.openstreetmap.org }",
   year = {2017},
 }

@article{mozafar2017simultaneous,
  title={A simultaneous approach for optimal allocation of renewable energy sources and electric vehicle charging stations in smart grids based on improved {GA}-{PSO} algorithm},
  author={M. R. Mozafar and M. H. Moradi and M. H. Amini},
  journal={Sustainable cities and society},
  volume={32},
  pages={627--637},
  year={2017},
  publisher={Elsevier}
}

@article{chang2021coordinate,
  title={Coordinate scheduling of electric vehicles in charging stations supported by microgrids},
  author={S. Chang and Y. Niu and T. Jia},
  journal={Electric Power Systems Research},
  volume={199},
  pages={107418},
  year={2021},
  publisher={Elsevier}
}

@article{tirunagari2022reaping,
  title={Reaping the benefits of smart electric vehicle charging and vehicle-to-grid technologies: Regulatory, policy and technical aspects},
  author={S. Tirunagari and M. Gu and L. Meegahapola},
  journal={IEEE Access},
  volume={10},
  pages={114657--114672},
  year={2022},
  publisher={IEEE}
}

@article{barman2023renewable,
  title={Renewable energy integration with electric vehicle technology: A review of the existing smart charging approaches},
  author={P. Barman and L. Dutta and S. Bordoloi and A. Kalita and P. Buragohain and S. Bharali and B. Azzopardi},
  journal={Renewable and Sustainable Energy Reviews},
  volume={183},
  pages={113518},
  year={2023},
  publisher={Elsevier}
}

@article{goke2022accounting,
  title={Accounting for spatiality of renewables and storage in transmission planning},
  author={L. G{\"o}ke and M. Kendziorski and C. Kemfert and C. Von Hirschhausen},
  journal={Energy Economics},
  volume={113},
  pages={106190},
  year={2022},
  publisher={Elsevier}
}

@article{brady2016development,
  title={Development of a driving cycle to evaluate the energy economy of electric vehicles in urban areas},
  author={J. Brady and M. O’Mahony},
  journal={Applied energy},
  volume={177},
  pages={165--178},
  year={2016},
  publisher={Elsevier}
}

@article{cole2021importing,
  title={Importing, outsourcing and pollution offshoring},
  author={M. A. Cole and R. J. R. Elliott and T. Okubo and L. Zhang},
  journal={Energy Economics},
  volume={103},
  pages={105562},
  year={2021},
  publisher={Elsevier}
}

@article{jakob2021carbon,
  title={Why carbon leakage matters and what can be done against it},
  author={M. Jakob},
  journal={One Earth},
  volume={4},
  number={5},
  pages={609--614},
  year={2021},
  publisher={Elsevier}
}

@article{will2024can,
  title={Can electric vehicle charging be carbon neutral? {U}niting smart charging and renewables},
  author={C. Will and F. Zimmermann and A. Ensslen and C. Fraunholz and P. Jochem and D. Keles},
  journal={Applied Energy},
  volume={371},
  pages={123549},
  year={2024},
  publisher={Elsevier}
}

@article{piao2022challenges,
  title={Challenges and development of {L}ithium-ion batteries for low temperature environments},
  author={N. Piao and X. Gao and H. Yang and Z. Guo and G. Hu and H. M. Cheng and F. Li},
  journal={Etransportation},
  volume={11},
  pages={100145},
  year={2022},
  publisher={Elsevier}
}

@article{jaguemont2016comprehensive,
  title={A comprehensive review of {L}ithium-ion batteries used in hybrid and electric vehicles at cold temperatures},
  author={J. Jaguemont and L. Boulon and Y. Dub{\'e}},
  journal={Applied Energy},
  volume={164},
  pages={99--114},
  year={2016},
  publisher={Elsevier}
}

@article{kambly2014estimating,
  title={Estimating the HVAC energy consumption of plug-in electric vehicles},
  author={K. R. Kambly and T. H. Bradley},
  journal={Journal of Power Sources},
  volume={259},
  pages={117--124},
  year={2014},
  publisher={Elsevier}
}

@article{liu2018exploring,
  title={Exploring the interactive effects of ambient temperature and vehicle auxiliary loads on electric vehicle energy consumption},
  author={K. Liu and J. Wang and T. Yamamoto and T. Morikawa},
  journal={Applied Energy},
  volume={227},
  pages={324--331},
  year={2018},
  publisher={Elsevier}
}

@article{donkers2020influence,
  title={Influence of driving style, infrastructure, weather and traffic on electric vehicle performance},
  author={A. Donkers and D. Yang and M. Viktorovi{\'c}},
  journal={Transportation Research Part D: Transport and Environment},
  volume={88},
  pages={102569},
  year={2020},
  publisher={Elsevier}
}

@inproceedings{valentina2014hvac,
  title={{HVAC} system modeling for range prediction of electric vehicles},
  author={R. Valentina and A. Viehl and O. Bringmann and W. Rosenstiel},
  booktitle={2014 IEEE Intelligent Vehicles Symposium Proceedings},
  pages={1145--1150},
  year={2014},
  organization={IEEE}
}

@article{liu2017impact,
  title={Impact of road gradient on energy consumption of electric vehicles},
  author={K. Liu and T. Yamamoto and T. Morikawa},
  journal={Transportation Research Part D: Transport and Environment},
  volume={54},
  pages={74--81},
  year={2017},
  publisher={Elsevier}
}

@article{madhusudhanan2020effect,
  title={Effect of a traffic speed based cruise control on an electric vehicleʼ s performance and an energy consumption model of an electric vehicle},
  author={A. K. Madhusudhanan and X. Na},
  journal={IEEE/CAA Journal of Automatica Sinica},
  volume={7},
  number={2},
  pages={386--394},
  year={2020},
  publisher={IEEE}
}

@article{liu2016modelling,
  title={Modelling the multilevel structure and mixed effects of the factors influencing the energy consumption of electric vehicles},
  author={K. Liu and J. Wang and T. Yamamoto and T. Morikawa},
  journal={Applied energy},
  volume={183},
  pages={1351--1360},
  year={2016},
  publisher={Elsevier}
}

@article{tang2015influences,
  title={Influences of the driver’s bounded rationality on micro driving behavior, fuel consumption and emissions},
  author={T. Q. Tang and H. J. Huang and H. Y. Shang},
  journal={Transportation Research Part D: Transport and Environment},
  volume={41},
  pages={423--432},
  year={2015},
  publisher={Elsevier}
}

@article{salari2023new,
  title={A new control algorithm of regenerative braking management for energy efficiency and safety enhancement of electric vehicles},
  author={A. H. Salari and H. Mirzaeinejad and M. F. Mahani},
  journal={Energy Conversion and Management},
  volume={276},
  pages={116564},
  year={2023},
  publisher={Elsevier}
}

@article{braun2017influence,
  title={The influence of driving patterns on energy consumption in electric car driving and the role of regenerative braking},
  author={A. Braun and W. Rid},
  journal={Transportation Research Procedia},
  volume={22},
  pages={174--182},
  year={2017},
  publisher={Elsevier}
}

@article{wu2022soc,
  title={{SOC} and {SOH} joint estimation of {L}ithium-ion battery based on improved particle filter algorithm},
  author={T. Wu and S. Liu and Z. Wang and Y. Huang},
  journal={Journal of Electrical Engineering and Technology},
  volume={17},
  number={1},
  pages={307--317},
  year={2022},
  publisher={Springer}
}

@article{wang2021review,
  title={A review on online state of charge and state of health estimation for {L}ithium-ion batteries in electric vehicles},
  author={Z. Wang and G. Feng and D. Zhen and F. Gu and A. Ball},
  journal={Energy Reports},
  volume={7},
  pages={5141--5161},
  year={2021},
  publisher={Elsevier}
}

@article{kajanova2022social,
  title={Social welfare-based charging of electric vehicles in the microgrids fed by renewables},
  author={M. Kajanova and P. Bracinik},
  journal={International Journal of Electrical Power and Energy Systems},
  volume={138},
  pages={107974},
  year={2022},
  publisher={Elsevier}
}

@article{soares2017dynamic,
  title={Dynamic electricity pricing for electric vehicles using stochastic programming},
  author={J. Soares and M. A. F. Ghazvini and N. Borges and Z. Vale},
  journal={Energy},
  volume={122},
  pages={111--127},
  year={2017},
  publisher={Elsevier}
}

@article{park2022electric,
  title={Electric vehicle charging management using location-based incentives for reducing renewable energy curtailment considering the distribution system},
  author={S. W. Park and K. S. Cho and G. Hoefter and S. Y. Son},
  journal={Applied Energy},
  volume={305},
  pages={117680},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{behrisch2011sumo,
  title={{SUMO}-simulation of urban mobility: an overview},
  author={M. Behrisch and L. Bieker and J. Erdmann and D. Krajzewicz},
  booktitle={Proceedings of SIMUL 2011, The Third International Conference on Advances in System Simulation},
  year={2011},
  organization={ThinkMind}
}

@inproceedings{kurczveil2014implementation,
  title={Implementation of an Energy Model and a Charging Infrastructure in SUMO},
  author={T. Kurczveil and P. {\'A}. L{\'o}pez and E. Schnieder},
  booktitle={Simulation of Urban Mobility: First International Conference, SUMO 2013, Berlin, Germany, May 15-17, 2013. Revised Selected Papers 1},
  pages={33--43},
  year={2014},
  organization={Springer}
}

@article{walpole2012weight,
  title={The weight of nations: an estimation of adult human biomass},
  author={S. C. Walpole and D. Prieto-Merino and P. Edwards and J. Cleland and G. Stevens and I. Roberts},
  journal={BMC public health},
  volume={12},
  pages={1--6},
  year={2012},
  publisher={Springer}
}

@article{millard2011we,
  title={Are we reaching peak travel? Trends in passenger transport in eight industrialized countries},
  author={A. Millard-Ball and L. Schipper},
  journal={Transport reviews},
  volume={31},
  number={3},
  pages={357--378},
  year={2011},
  publisher={Taylor \& Francis}
}



@misc{CiteEursotatMobility,
  title={Passenger mobility statistics},
  author={Eurostat},
  year={2021},
  howpublished = {\url{https://ec.europa.eu/eurostat/statistics-explained/index.php?title=Passenger_mobility_statistics#Passenger_car_occupancy}}
}

@misc{TomTomODAnalysis,
  title={Tom{T}om {OD} Matrix Analysis},
  author={TomTom},
  year={2022},
  howpublished = {\url{https://www.tomtom.com/products/origin-destination-matrix-analysis/}}
}

@article{al2022effects,
  title={Effects of ambient temperature and trip characteristics on the energy consumption of an electric vehicle},
  author={Y. Al-Wreikat and C. Serrano and J. R. Sodr{\'e}},
  journal={Energy},
  volume={238},
  pages={122028},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{unni2021influence,
  title={Influence of Auxiliary Loads on the Energy Consumption of Electric Vehicle--A Case Study},
  author={K. Unni and S. Thale},
  booktitle={2021 IEEE Transportation Electrification Conference (ITEC-India)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}

@article{sun2021energy,
  title={Energy consumption simulation and economic benefit analysis for urban electric commercial-vehicles},
  author={D. J. Sun and Y. Zheng and R. Duan},
  journal={Transportation Research Part D: Transport and Environment},
  volume={101},
  pages={103083},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{evtimov2017energy,
  title={Energy consumption of auxiliary systems of electric cars},
  author={I. Evtimov and R. Ivanov and M. Sapundjiev},
  booktitle={MATEC web of conferences},
  volume={133},
  pages={06002},
  year={2017},
  organization={EDP Sciences}
}

@book{urry2014offshoring,
  title={Offshoring},
  author={J. Urry},
  year={2014},
  publisher={Wiley}
}


@book{Bernardo:1319894,
  author = {J. M. Bernardo and A. Smith},
      title         = "{Bayesian Theory}",
      publisher     = "Wiley",
      series        = "Wiley series in probability and statistics",
      year          = "2000",
}

@book{Tanner1996,
  author = {M. Tanner},
   publisher = {Springer},
  title = {Tools for statistical inference},
  year = {1996}
}

@book{AP91,
    author = {{A. Papoulis}},
  publisher = {McGraw-Hill},
  title = {Probability, random variables, and stochastic processes},
  year = {1991}
}
.

@inproceedings{forget,
  title={Bayesian Estimation of Non-stationary {AR} Model Parameters via an Unknown Forgetting Factor},
  author={V. \v{S}m\'{\i}dl and A. Quinn},
  booktitle={Proc. IEEE Workshop on Dig. Sig. Process.},
  pages={221-225},
  year={2004},
  organization={IEEE}
}
